Holographic Renormalization Group and Stress Tensor Operators

The holographic duality conjectures a relation between strongly coupled quantum systems and quantum gravity in higher-dimensional spacetimes. Gravitational theories in two and three dimensions are meaningful examples for classical and quantum exploration due to their unique characteristics, notably the absence of propagating bulk degrees of freedom and the presence of only boundary degrees of freedom, distinguishing them from higher-dimensional counterparts. These gravitational theories exhibit complex interactions when the bulk spacetime has a finite size, regulated by Zamolodchikov's double-trace irrelevant $T\overline{T}$ operator. This thesis aims to gain a holographic understanding of $\mathrm{AdS}_3$ and JT gravity under the influence of the $T\overline{T}$ deformation. Under a finite radial cutoff, these theories exhibit perturbative behavior that implies the emergence of the Nambu-Goto action for the corresponding boundary graviton action. We also conducted semi-classical calculations of observables related to finite-cutoff gravity and its dual $T\overline{T}$-deformed CFT description, including correlation functions involving stress tensors and gravitational Wilson lines, along with an analysis of their supersymmetric extensions. Additionally, we explored the implications of general stress tensor deformations within field-theoretic and holographic settings. This thesis integrates previously adapted publications while also pioneering new ground, notably exploring the definition of a quantum $T\overline{T}$ operator beyond two dimensions with $\frac{1}{N}$ corrections, investigating quantum-corrected higher point correlators for a planar boundary, and offering insights into a two-dimensional spherical boundary at a finite cutoff. Furthermore, throughout the thesis, we show more details in calculations at various points.

==> Makefile <==

#
# uclathes Makefile
# Copyright (C) 1995 by John Heidemann, <johnh@isi.edu>
#

FILES=README \
	demo.tex demo.dvi demo.ps \
	demo2big.tex demo2mac.tex demo2rep.tex demo2the.tex demo2int.tex demo2ti.tex demo2rep.ps demo2the.ps \
	thesdoc.tex thesdoc.ps \
	uclathes.cls uclath12.clo uclathti.clo uclathma.clo \
	uclathes.bst Makefile

all:  latex dvips

tar: $(FILES)
	tar cvf uclathes.tar $(FILES)

tar.gz:
	@echo "Make all before doing make tar.gz"
	tar czvf uclathes.tar.gz $(FILES)

latex: latex.demo latex.demo2rep latex.demo2the latex.thesdoc

dvips: dvips.demo dvips.demo2rep dvips.demo2the dvips.thesdoc

latex.demo:
	latex demo

dvips.demo:
	dvips demo

latex.demo2rep:
	latex demo2rep

dvips.demo2rep:
	dvips demo2rep

latex.demo2the:
	latex demo2the

dvips.demo2the:
	dvips demo2the

latex.thesdoc:
	latex thesdoc

dvips.thesdoc:
	dvips thesdoc



